InteractRank: Personalized Web-Scale Search Pre-Ranking with Cross Interaction Features

Modern search systems use a multi-stage architecture to deliver personalized results efficiently. Key stages include retrieval, pre-ranking, full ranking, and blending, which refine billions of items to top selections. The pre-ranking stage, vital for scoring and filtering hundreds of thousands of items down to a few thousand, typically relies on two tower models due to their computational efficiency, despite often lacking in capturing complex interactions. While query-item cross interaction features are paramount for full ranking, integrating them into pre-ranking models presents efficiency-related challenges. In this paper, we introduce InteractRank, a novel two tower pre-ranking model with robust cross interaction features used at Pinterest. By incorporating historical user engagement-based query-item interactions in the scoring function along with the two tower dot product, InteractRank significantly boosts pre-ranking performance with minimal latency and computation costs. In real-world A/B experiments at Pinterest, InteractRank improves the online engagement metric by 6.5% over a BM25 baseline and by 3.7% over a vanilla two tower baseline. We also highlight other components of InteractRank, like real-time user-sequence modeling, and analyze their contributions through offline ablation studies. The code for InteractRank is available at https://github.com/pinterest/atg-research/tree/main/InteractRank.

==> www_25/interaction-features.tex <==
\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */}
\begin{algorithm}[bt]

\caption{Algorithm for computing Cross Interaction Features}\label{alg:two}
\KwData{$Q \gets$ Queries, $I \gets$ Items}
\KwData{$\lambda \gets$ engagement threshold, ${imp} \gets$  impressions, $s \gets$ saves, $lc \gets$ long clicks, $w \gets$ weight}
\KwData{ $P \gets$ Perf Metrics, $AP \gets$ Aggregated ItemPerf metrics, $IP \gets$ ItemPerf score, $QP \gets$ QueryPerf score, $IQP \gets$ <Query, Items, ItemQueryPerf Score>}
\For{$q \in Q$}{
    {$AP_q \gets \emptyset$;}
    {$QP_q \gets \emptyset$;}

    \For{$i \in I$}{
        \If{$P_{i}$ exists}
                {$AP_{i}  = P_{i_{existing}} + P_{i_{new}} * w$ \\
                }
         \Else
         {$AP_{i}  = P_{i_{existing}}$}
        {$QP_q = QP_q + P_{i_{new}} * w$ } \\
        {$AP_q$ \cup <i, $AP_i$>}
    }
{$IP \gets \emptyset$;} \\
\For{<i, $AP> \in AP_q$} {
{$IP_i = \frac{(AP_s + (w_{lc} * AP_{lc}))}{AP_{imp}}$} \\
{$IP$ \cup <$i$ , $IP_i>$}
} \\
\If{$QP_{imp} \leq \lambda$}
            {continue;} \\
{$Q_{q_{score}} = \frac{(QP_s + (w_{lc} * QP_{lc}))}{QP_{imp}}$}

 {$IQP \gets \emptyset$;} \\
\For{<$i,\, $IP_i$> \in IP$} { 
  {$IQP_i = 2 \sigma \left(\frac{IP_{i}}{\max({0.1,  Q_{q_{score}}})}\right) - 1$} \\ 
    {$IQP$ \cup <$q$, $i$, $IQP_i$>}
    }
   
}
\end{algorithm}
